Linear smoothed extended finite element method

The extended finite element method (XFEM) was introduced in 1999 to treat problems involving discontinuities with no or minimal remeshing through appropriate enrichment functions. This enables elements to be split by a discontinuity, strong or weak and hence requires the integration of discontinuous functions or functions with discontinuous derivatives over elementary volumes. Moreover, in the case of open surfaces and singularities, special, usually non-polynomial functions must also be integrated. A variety of approaches have been proposed to facilitate these special types of numerical integration, which have been shown to have a large impact on the accuracy and the convergence of the numerical solution. The smoothed extended finite element method (SmXFEM) [1], for example, makes numerical integration elegant and simple by transforming volume integrals into surface integrals. However, it was reported in [1, 2] that the strain smoothing is inaccurate when non-polynomial functions are in the basis. This is due to the constant smoothing function used over the smoothing domains which destroys the effect of the singularity. In this paper, we investigate the benefits of a recently developed Linear smoothing procedure [3] which provides better approximation to higher order polynomial fields in the basis. Some benchmark problems in the context of linear elastic fracture mechanics (LEFM) are solved to compare the standard XFEM, the constant-smoothed XFEM (Sm-XFEM) and the linear-smoothed XFEM (LSm-XFEM). We observe that the convergence rates of all three methods are the same. The stress intensity factors (SIFs) computed through the proposed LSm-XFEM are however more accurate than that obtained through Sm-XFEM. To conclude, compared to the conventional XFEM, the same order of accuracy is achieved at a relatively low computational effort.

==> xfemIntro.tex <==
\section{Overview of the extended finite element method}
%\subsection{Partition of unity}
The mathematical ideas of XFEM are based on the Partition of unity finite element methods (PUFEM) which were first discussed in \cite{babuvska1997partition, melenk1996partition}. The partition of unity refers to any set of function $N_I(\bf{x})$ which has the following two properties
\begin{itemize}
\item Summation of the function with in its domain is unity
%Eq 20
\begin{equation}
\sum_{I=1}^n\limits N_I(\bf{x}) = 1
\label{eq19}
\end{equation}
\item When operated on a function $f(\bf{x})$, it would reproduce the same function $f(\bf{x})$ with in the domain
%Eq 21
\begin{equation}
\sum_{I=1}^n\limits N_I(\bf{x})f(\bf{x}) = f(\bf{x})
\label{eq20}
\end{equation}
\end{itemize}
The basic idea is to embed the local nature of the solution by using the partition of unity framework. This is usually best obtained by using the conforming ansatz spaces with apriori knowledge of the solution \cite{babuvska1997partition}. The effect of the ansatz functions vanishes towards the element boundaries when multiplied with the partition of unity functions. Hence the local nature of the enrichment function is preserved. These approximation functions may be polynomials, harmonic functions or singular functions depending on the problem under consideration. However, care should be taken in the integration of these functions as they are likely to have steep gradients.

\subsection{Enrichment functions}
Enrichment functions as mentioned earlier, are highly case specific and are used to arrive at the required localised approximation to the solution. Enrichments are of two types namely, intrinsic enrichments and extrinsic enrichments. Intrinsic enrichments are those which do not require additional degrees of freedom to represent the field of interest. Fries and Belytschko \cite{fries2006intrinsic} proposed this method. Only the basis function will be modified to reproduce the exact analytical solution which is known a priori. Let $U^h(\bf{x})$ be the assumed trial function, $\bf{u}^T$ be the basis vector used globally and $\bf{a}$ is the nodal values of the solution. The displacement field is then given by Equation\eqref{eq21}. 

%Eq 22
\begin{equation}
U^h(\bf{x})={\bf{u}^T}\bf{a}
\label{eq21}
\end{equation}
For a linear displacement field the basis is given by Equation\eqref{eq22}. 
%Eq 23
\begin{equation}
\begin{aligned}
\bf{u^T}&=
\begin{Bmatrix}
1 & x & y
\end{Bmatrix}\\
\end{aligned}
\label{eq22}
\end{equation}
If we are to get a better approximation we can add more terms to the basis vector as given in Equation\eqref{eq23}. They can be higher order polynomials, harmonic functions, logarithmic functions etc.
%Eq 24
\begin{equation}
\begin{aligned}
\bf{u^T_{enr}}&=
\begin{Bmatrix}
1 & x & y & F_m
\end{Bmatrix}\\
\end{aligned}
\label{eq23}
\end{equation}
In LEFM, approximation space can be spanned by the crack tip the enrichment terms \cite{babuvska1997partition} given by Equation\eqref{eq24}
%Eq 25
\begin{equation}
\begin{aligned}
F_m&=
\begin{Bmatrix}
\sqrt{r}\sin\dfrac{\theta}{2} & \sqrt{r}\cos\dfrac{\theta}{2} &
\sqrt{r}\sin\theta \sin\dfrac{\theta}{2} & \sqrt{r}\sin\theta \cos\dfrac{\theta}{2}
\end{Bmatrix}\\
\end{aligned}
\label{eq24}
\end{equation}
Hence for intrinsic enrichment the enriched approximation basis is given by Equation\eqref{eq25}
%Eq 26
\begin{equation}
\begin{aligned}
\bf{u^T_{enr}}&=
\begin{Bmatrix}
1 & x & y & \sqrt{r}\sin\dfrac{\theta}{2} & \sqrt{r}\cos\dfrac{\theta}{2} &
\sqrt{r}\sin\theta \sin\dfrac{\theta}{2} & \sqrt{r}\sin\theta \cos\dfrac{\theta}{2}
\end{Bmatrix}\\
\end{aligned}
\label{eq25}
\end{equation}
Extrinsic enrichments are the more commonly used enrichments which use additional basis vectors which are associated with additional degrees of freedom.
%Eq 27
\begin{equation}
U^h(\mathbf{x})=\sum_{I\in \mathscr{N}^{std}}\limits \mathbf{N}_I \mathbf{u}_I+
  	   \sum_{J\in \mathscr{N}^{hev}}\limits \mathbf{N}_J H(\mathbf{x}) \mathbf{a}_J+
       \sum_{K\in \mathscr{N}^{tip}}\limits \mathbf{N}_K \left( \sum_{m=1}^4 \limits F_m(\mathbf{x}) \mathbf{b}_K^m\right) 
\label{eq26}
\end{equation}
where $I$ is the set of all the nodes in the system, $J$ is the set of nodes which are completely cut by the crack, $K$ is the set of nodes which contain the crack tips as shown in Figure \ref{xfem_discrete}. $\mathbf{N}_I(\mathbf{x})$ are the standard shape functions associated with the standard DOF $\mathbf{u}_I$ , $H(\mathbf{x})$ are the Heaviside functions associated with the enriched DOF, $\mathbf{a}_J$ and $F_m$ are the tip enrichment functions associated with the DOF, $\mathbf{b}_K^m$. Since the first term of Equation \eqref{eq24} is already a discontinuous function it will not be used in combination with the Heaviside function. Hence the tip element will contain only the asymptotic enrichment terms. Only those elements which contain these enriched nodes will have the effect of enrichment. Hence there will be some elements with all nodes enriched and some elements with only some nodes enriched, the so called ‘blending elements’ which need special attention to get accurate results. Heaviside (for complete strong discontinuity) enrichments are used in order to represent the jump across the discontinuity. If the displacement field of the form in Equation \eqref{eq27} is used it will lead to spurious enrichment contribution to standard nodes. This failure in interpolation can be corrected by a simple shifting of the Heaviside function as proposed in \cite{belytschko2001arbitrary} and the correct values can be recovered at the nodes. The modified field is given by Equation \eqref{eq27}
%Eq 28
\begin{equation}
U^h(\mathbf{x})=\sum_{I\in \mathscr{N}^{std}}\limits \mathbf{N}_I \mathbf{u}_I+
  	   \sum_{J\in \mathscr{N}^{hev}}\limits \mathbf{N}_J \left( H(\mathbf{x})-H(\mathbf{x}_J) \right) \mathbf{a}_J+
       \sum_{K\in \mathscr{N}^{tip}}\limits \mathbf{N}_K \left( \sum_{m=1}^4 \limits \left( F_m(\mathbf{x})-F_m(\mathbf{x}_K) \right) \mathbf{b}_K^m\right)
\label{eq27}
\end{equation}
By this correction the effect of the enrichment on the boundary vanishes on all fully enriched elements. Another method is also given in \cite{fries2008corrected} to correct this error in interpolation.
\begin{figure}
\centering
\includegraphics[width=0.7\textwidth]{./Figures/xfem.eps}
\caption{XFEM discretisation of cracked domain}
\label{xfem_discrete}
\end{figure}

\subsection{Numerical integration}
Once displacement field is approximated based on the above mentioned procedure, we end up with the familiar system of linear equations
%Eq 29
\begin{equation}
\mathbf{K}\mathbf{U}^h=\mathbf{F}
\label{eq28}
\end{equation}
where
%Eq 30
\begin{equation}
\mathbf{K}^e=
\begin{bmatrix} 
%K_{ij}^{uu} & K_{ij}^{ua} & K_{ij}^{ub}\\
%K_{ij}^{au} & K_{ij}^{aa} & K_{ij}^{ab}\\
%K_{ij}^{bu} & K_{ij}^{ba} & K_{ij}^{bb}
\mathbf{K}^{uu} & \mathbf{K}^{ua} & \mathbf{K}^{ub}\\
\mathbf{K}^{au} & \mathbf{K}^{aa} & \mathbf{K}^{ab}\\
\mathbf{K}^{bu} & \mathbf{K}^{ba} & \mathbf{K}^{bb}
\end{bmatrix}
\label{eq29}
\end{equation}
where, the superscript $uu$ refers to standard FEM components, $ua$ refers to cross components of standard FEM and the Heaviside enrichment terms, $ub$ refers to the cross components of standard FEM and the asymptotic enrichment terms and other terms can be defined similarly. The formulation of the constituents of the above element matrix and the implementation aspects of XFEM can be found in references \cite{mohammadi2008extended} and \cite{pommier2013extended}.

Though XFEM significantly reduces the modelling and computational effort for moving boundary problems,the low computational effort comes at the cost of accuracy of the solution. The problem associated with XFEM is with the numerical integration of the singular functions involved. The difficulty in numerical integration is that the discontinuous functions cannot be integrated with good accuracy using the Gauss quadrature rule as it implicitly assumes a polynomial approximation. One solution is to use higher order Gauss quadrature as suggested in \cite{bechet2005improved} and \cite{laborde2005high}. Moes et al. \cite{dolbow1999finite} suggested the use of subcells. The elements that are intersected by the discontinuity are further subdivided into quadrilaterals (sub-quads) or triangles (sub-triangles) based on the geometry. But it is done such that these sub cells share the discontinuity as one of their edges. It is to be noted that this subdivision is merely for the purpose of integration and it does not associate any additional DOF with the element. The scheme provided by Fish \cite{fish1989finite} also performs adequately. They used simple trapezoids instead. Sukumar et al. \cite{sukumar2000extended} also extended the subcell methods for use in three dimensional problems with discontinuity. Ventura \cite{ventura2006elimination} proposed a new method for integration of discontinuous functions. In this method there is no need for subdividing the cut elements into subcells. The basic idea was to recast the integrand functions into equivalent polynomials which are continuous and differentiable in the domain. As they are continuous they can be easily integrated by normal Gauss integration scheme. In \cite{ventura2009fast} the enrichment function is pre-multiplied with a smoothing function. The smoothing takes care of the problem of blending elements as well. This method is similar to the SFEM techniques, but in this method there is a constraint on the enriched degrees of freedom associated with the crack tip enrichment to be equal. The present scheme does not pose any such constraints. Natarajan et al. \cite{natarajan2009numerical} numerically integrated arbitrary polygons based on Schwarz-Christoffel conformal mapping. This method reduces the two level iso-parametric mapping introduced by Sukumar and Tabarraei \cite{sukumar2004conforming} to one level. The methods applications can also be found in \cite{natarajan2010integrating}
